Towards data-driven stroke rehabilitation via wearable sensors and deep learning

Recovery after stroke is often incomplete, but rehabilitation training may potentiate recovery by engaging endogenous neuroplasticity. In preclinical models of stroke, high doses of rehabilitation training are required to restore functional movement to the affected limbs of animals. In humans, however, the necessary dose of training to potentiate recovery is not known. This ignorance stems from the lack of objective, pragmatic approaches for measuring training doses in rehabilitation activities. Here, to develop a measurement approach, we took the critical first step of automatically identifying functional primitives, the basic building block of activities. Forty-eight individuals with chronic stroke performed a variety of rehabilitation activities while wearing inertial measurement units (IMUs) to capture upper body motion. Primitives were identified by human labelers, who labeled and segmented the associated IMU data. We performed automatic classification of these primitives using machine learning. We designed a convolutional neural network model that outperformed existing methods. The model includes an initial module to compute separate embeddings of different physical quantities in the sensor data. In addition, it replaces batch normalization (which performs normalization based on statistics computed from the training data) with instance normalization (which uses statistics computed from the test data). This increases robustness to possible distributional shifts when applying the method to new patients. With this approach, we attained an average classification accuracy of 70%. Thus, using a combination of IMU-based motion capture and deep learning, we were able to identify primitives automatically. This approach builds towards objectively-measured rehabilitation training, enabling the identification and counting of functional primitives that accrues to a training dose.

==> tables/best_hype_params.tex <==
\begin{table}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Statistical features} & \multicolumn{3}{c|}{Features learned from raw signal} \\ \hline
\begin{tabular}[c]{@{}c@{}}Random \\ forest\end{tabular} & \begin{tabular}[c]{@{}c@{}}Fully \\ connected \\ neural \\ network\end{tabular} & CNN & LSTM & \begin{tabular}[c]{@{}c@{}}Proposed\\ model\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}Min. sample(s)\\  at leaf = 1\\  Min. samples \\ at split = 20\end{tabular} & \begin{tabular}[c]{@{}c@{}}\# of \\ hidden units \\ = 900\\ \# of \\ layers = 8\end{tabular} & \begin{tabular}[c]{@{}c@{}}Arch: DenseNet-style\\ Normalization: BN\\ Embedding \\ for sensors: No\end{tabular} & \begin{tabular}[c]{@{}c@{}}Dim. of \\ hidden \\ unit\\  = 4000\end{tabular} & \begin{tabular}[c]{@{}c@{}}Arch: ResNet-style\\ Normalization: IN\\ Embedding \\ for sensors: Yes\end{tabular} \\ \hline
\end{tabular}
\caption{The best performing hyperparameters for all the models. Between the two variants of RNN, we report the hyper-parameters only for the variant that performs the best (i.e. LSTM). }
\label{tab:best_hype_params}
\end{table}

==> tables/model_comp_test_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\begin{tabular}{|c|c|c|c|c|}
\hline
Models & Model type & Best model configuration & \begin{tabular}[c]{@{}c@{}}Test \\ accuracy \\ (balanced)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Test \\ accuracy\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Statistical \\ feature-based \\ models\end{tabular}} & Random forest & \begin{tabular}[c]{@{}c@{}}Min. sample(s) at leaf = 1\\ Min. samples at split = 20\end{tabular} & 52.66 & 59.40 \\ \cline{2-5} 
 & \begin{tabular}[c]{@{}c@{}}Fully connected \\ neural network\end{tabular} & \begin{tabular}[c]{@{}c@{}}\# of hidden units = 900\\ \# of layers = 8\\ Dropout = 0.5\end{tabular} & 58.04 & 62.43 \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Model where\\  features\\  are learned \\ from raw data\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Traditional conv.\\  network\end{tabular} & \begin{tabular}[c]{@{}c@{}}Arch: DenseNet-style\\ Normalization: BN\\ Embedding for sensors: No\end{tabular} & 64.01 & 64.98 \\ \cline{2-5} 
 & Bi - LSTM & Hidden unit dim. = 1200 & 63.92 & 65.13 \\ \cline{2-5} 
 & LSTM & Hidden unit dim. = 4000 & 66.58 & 68.21 \\ \cline{2-5} 
 & Proposed Model & \begin{tabular}[c]{@{}c@{}}Arch: ResNet-style\\ Normalization: IN\\ Embedding for sensors: Yes\end{tabular} & 69.21 & 70.67 \\ \cline{2-5}
 & Ensemble Model & \begin{tabular}[c]{@{}c@{}}Combined LSTM\\  and Proposed Model\end{tabular} & 70.11 & 71.87 \\
 \hline
\end{tabular}
\caption{The table shows performance of best models with various learning strategies.}
\label{tab:final_results_table}
\end{table}

==> tables/only_bacc_sev_pat.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Model\\ type\end{tabular} & \begin{tabular}[c]{@{}c@{}}Random \\ forest\end{tabular} & FCNN & \begin{tabular}[c]{@{}c@{}}Traditional \\ CNN\end{tabular} & LSTM & \begin{tabular}[c]{@{}c@{}}Proposed\\ model\end{tabular} & Ensemble \\ \hline
\begin{tabular}[c]{@{}c@{}}Balanced\\ accuracy\end{tabular} & 32.90 & 36.60 & 38.22 & 41.76 & 43.50 & \textbf{44.39} \\ \hline
\end{tabular}
\caption{Balanced accuracies for different models described in Section \ref{sec:computational_exp} for severe patients. Although the performance drops for all the models, the ensemble model and the proposed model are still the best performing models.(FCNN = Fully connected neural network, Ensemble = Proposed model + LSTM)}
\label{tab:severe_set_bacc}
\end{table}

==> tables/performance_on_severe_pats.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\begin{tabular}{|c|c|c|c|c|}
\hline
Models & Model type & Best model configuration & \begin{tabular}[c]{@{}c@{}}Test \\ accuracy \\ (balanced)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Test \\ accuracy\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Statistical \\ feature-based \\ models\end{tabular}} & Random forest & \begin{tabular}[c]{@{}c@{}}Min. sample(s) at leaf = 1\\ Min. samples at split = 20\end{tabular} & 32.90 & 33.89 \\ \cline{2-5} 
 & \begin{tabular}[c]{@{}c@{}}Fully connected \\ neural network\end{tabular} & \begin{tabular}[c]{@{}c@{}}\# of hidden units = 900\\ \# of layers = 8\\ Dropout = 0.5\end{tabular} & 36.60 & 39.62 \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Model where\\  features\\  are learned \\ from raw data\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Traditional conv.\\  network\end{tabular} & \begin{tabular}[c]{@{}c@{}}Arch: DenseNet-style\\ Normalization: BN\\ Embedding for sensors: No\end{tabular} & 38.22 & 43.11 \\ \cline{2-5} 
 & Bi - LSTM & Hidden unit dim. = 1200 & 38.22 & 42.57 \\ \cline{2-5} 
 & LSTM & Hidden unit dim. = 4000 & 41.76 & 48.78 \\ \cline{2-5} 
 & Proposed Model & \begin{tabular}[c]{@{}c@{}}Arch: ResNet-style\\ Normalization: IN\\ Embedding for sensors: Yes\end{tabular} & 43.50 & 44.44 \\ \cline{2-5}
 & Ensemble Model & \begin{tabular}[c]{@{}c@{}}Combined LSTM\\  and Proposed Model\end{tabular} & 44.39 & 48.36 \\
 \hline
\end{tabular}
\caption{The table shows performance of best models with various learning strategies.}
\label{tab:final_results_table}
\end{table}
